Heuristic-Based Weak Learning for Automated Decision-Making

Machine learning systems impact many stakeholders and groups of users, often disparately. Prior studies have reconciled conflicting user preferences by aggregating a high volume of manually labeled pairwise comparisons, but this technique may be costly or impractical. How can we lower the barrier to participation in algorithm design? Instead of creating a simplified labeling task for a crowd, we suggest collecting ranked decision-making heuristics from a focused sample of affected users. With empirical data from two use cases, we show that our weak learning approach, which requires little to no manual labeling, agrees with participants' pairwise choices nearly as often as fully supervised approaches.

==> modules/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Broadly, weakly supervised learning combines the ``top-down" and ``bottom-up" approaches to moral decision-making. This approach significantly reduces the costs associated with obtaining large sets of high-quality labels while retaining out-of-sample accuracy. Sourcing moral principles from experts provides advantages for customizing domain-specific algorithms without requiring the rigid, disjunctive set of rules need to code a game-theoretic model; it is unreasonable to assume that a set of non-conflicting moral principles can be obtained for any sufficiently complex moral problem, and heuristic functions are expected to overlap and conflict. My approach does not attempt to create a unified moral theory; rather, experts can provide just as much heuristic information as they have about the domain without attempting to generalize beyond their contingent experience; in this way, moral expertise from multiple specialists can be combined to create an efficient moral decision-maker across the entire domain. Additionally, in the fully-supervised case, domain experts have no way to express uncertainty in their moral decisions. In semi-supervision, probabilistic labels confer the relative uncertainty of the heuristics about a given moral decision to the discriminative model, which makes the final, discrete decision based on generalizations across multiple, uncertain labels. 

My approach also has the logistical advantage of interfacing with machine learning at the training phase. Rather than adding a new suite of moral models to their machine learning pipelines, practitioners can use existing classification techniques trained on the combined labels provided by experts' moral heuristics. For the purposes of interpretability, the output of the label model can be accounted for by examining the individual votes of each heuristic function. Interpretations at the discriminative step must be obtained using existing interpretability methods, or a naturally interpretable classifier (such as a decision tree) \citep{Du2018TechniquesLearning}.

The experiments performed in Section \ref{sec:experiments} show that while heuristics derived from measured moral preferences do not always agree with survey respondents, a weakly-supervised machine learning approach can make comparable moral decisions with no crowdsourcing whatsoever. Though this paper uses crowd-sourced data to prove the efficacy of my method, this approach does not require massive data collection. In a real-world example, a set of experts need only provide a set of heuristics and a small development set of hand-labeled dilemmas for validation. For simpler domains, I show that finding a small set of popular heuristics and asking respondents to rank those heuristics may be a viable alternative to collecting a full set of pairwise comparisons, and may in fact capture more information about the relative certainty of respondents' moral decisions. Surveys may not be even necessary; one potential application of this approach is to search an external knowledge base, such as a body of law, for heuristics relevant to a given moral dilemma and write heuristics using those legal principles. Ethical recommendations, commonly carefully constructed and released by watchdogs, also constitute a fruitful source of moral heuristics \citep{Luetge2017TheDriving}.

Theoretically, this approach is not limited to cheaply replicating the preferences of experts, scholars, lawyers, and crowds. Heuristics are especially useful for breaking down complex problems into sub-problems that can be solved with shortcuts or approximations. As a proof-of-concept, this investigation was limited to domains where moral preference data already exists. I hope that future work will attempt to elicit and validate heuristics from domain experts to solve a real-world moral dilemma in more complex domains without easily measured moral preferences. In these domains, the heuristic approach may be the only viable framework for making moral decisions.

However, there are still important problems to solve before moral decision-making algorithms are truly reliable. First, the problem of representation is ignored; heuristic functions can only operate on a set of measurable, observable features selected by domain engineers to have moral status. This framework mitigates the representation problem by relying on experts, who may be informed enough to handle extremely detailed feature sets, but representations may still aggressively reduce the dilemma at hand. Hierarchical feature representations might provide a useful interface for combining the expertise of individuals in different fields of a particular domain; an expert might be able to specify very granular heuristics for one set of features, but may only be able to express broad heuristics for less-familiar areas of the feature space. 

Second, experts must be selected carefully; issues of selection bias and small sample sizes could create poorly specified heuristic functions or systematically disadvantage underrepresented groups. For example, the best-performing heuristic writers in a Snorkel workshop were individuals with an M.S. or a Ph.D. and strong Python coding skills \citep{Ratner2017Snorkel:Supervision}. To incorporate multiple perspectives, some level of translation between domain experts without a high level of education and coding skill is required. Oversight is also important for accountability; future work should focus on designing human-in-the-loop workflows for interpreting moral decisions and adjusting heuristics accordingly. In general, the risk of systematic error increases as fewer perspectives are consulted; but crowd-sourcing is not the only way to solve this problem, as I demonstrate with the ranked-choice experiment. Crucially, this framework depends wholly on the moral expertise of the heuristic writers and their ability to represent the interests of stakeholders in the domain. In other words, if a crowdsourcing approach is democratic and a ``top-down" approach is totalitarian, then this approach relies on a representative democracy to reach acceptable moral outcomes, with all the ensuing trade-offs. 

Perhaps the most useful avenue of future work is the incorporation of moral heuristics with amoral or domain-specific optimization objectives. This investigation deals only with isolated moral dilemmas, in which the moral decision has been isolated from other optimizations in the problem. (For instance, in the kidney exchange, moral decisions are made only in the case of a tie; moral factors are not considered in the rest of the matching algorithm.) But because this framework operates at the labeling stage, it could be integrated as a secondary or superseding label ground-truth during training. With a set of moral heuristics, an autonomous vehicle might act differently if it encountered a deer in the road than it would if it encountered some inanimate obstacle.








==> modules/problem.tex <==
\section{Problem Statement}
\label{sec:problem}

The field of algorithmic ethics has a long history and a broad set of problems \citep{Moor1985WhatEthics}. This paper deals in particular with moral dilemmas, scenarios in which an agent faced with multiple alternatives is morally compelled to choose each, but can only choose one \citep{Sinnott-Armstrong1988MoralDilemmas, Yu2018BuildingIntelligence}. For instance, an autonomous vehicle in the Moral Machine problem is morally compelled to save both the passengers and the pedestrians, but due to brake failure or some other physical constraint must choose which group to save. Formally, let $\mathcal{A}$ be a finite set of possible alternatives, where each alternative is represented by a vector of relevant moral or situational features. An instance of a moral dilemma consists of a set of alternatives $X \in \mathcal{A}$ of size $K$ such that a moral agent is compelled to choose (not choose) each alternative but must choose only one. An answer to the dilemma takes the form of an ordinal ranking $y$ over $X$ which ranks the moral appeal of each alternative.

In addition to the trolley dilemma for autonomous vehicles, there are many scenarios in which an automated agent or algorithm may face a moral dilemma, especially when interacting with human beings: when two matches for a donor kidney are found, which patient should receive the kidney? Is a repentant convict more deserving of parole than an unrepentant one? Should an advertising algorithm consider the moral impacts of particular advertisements on particular users? Moral dilemmas are usually reserved for human judgment, but as algorithms are endowed with more and more responsibility in human affairs, they will inevitably face moral dilemmas that are either too immediate, too minute, or too complicated to be left to human judgment. As a result, some researchers have called for a general framework for automated moral decision-making \citep{Conitzer2017MoralIntelligence}.

\begin{inparaenum}[(1)]
There are several important problems to solve when automating ethical decision-making. \item\label{rep} To specify a moral dilemma, researchers must choose a representation of all relevant considerations, or features, for each alternative. In the Moral Machine experiment, features include inter alia age, gender, and class status. Features must be specific enough to convey meaningful information about the moral factors at play, but general enough to be decipherable by a domain expert or a layperson for coding or training the model. Oversimplification of the problem into only a few moral features, as is often necessary in experiments intended to measure moral preferences, may miss crucial factors that should influence decision-making. \item\label{sem} The moral agent must learn or operate according to semantic knowledge of moral principles or preferences. \item\label{conflict} In the absense of clear moral consensus, the agent must be pluralistic; that is, it must reconcile multiple moral principles or preferences. \item\label{inter} The moral agent's decisions should be interpretable. If the agent has moral responsibility, there must be a way to account for its decisions to affected users, for ethical and regulatory reasons. For this reason, the use of black box models for moral decision-making is somewhat unappealing unless the model is made sufficiently interpretable \citep{Du2018TechniquesLearning}. Section~\ref{sec:background} reviews some contemporary solutions to these problems and their shortcomings.
\end{inparaenum}

==> modules/title.tex <==
\begin{titlepage}
\singlespacing

\begin{center}

\vspace*{.06\textheight}
{\scshape\LARGE\color{primary} \univname\par}\vspace{1.5cm} % University name
\textsc{\Large Undergraduate Thesis}\\[0.5cm] % Thesis type

\par\noindent\rule{\textwidth}{1pt}\\[0.4cm]
{\LARGE \bfseries \ttitle\par}\vspace{0.4cm} % Thesis title
\par\noindent\rule{\textwidth}{1pt}\\[1.5cm]
 
\begin{minipage}[t]{0.4\textwidth}
\begin{flushleft} \large
\emph{Author:}\\
{\color{primary} \authorname} % Author name - remove the \href bracket to remove the link
\end{flushleft}
\end{minipage}
\begin{minipage}[t]{0.4\textwidth}
\begin{flushright} \large
\emph{Comittee:} \\
{\color{primary} {\chair} (Chair)}\\{\comittee} % Supervisor name - remove the \href bracket to remove the link  
\end{flushright}
\end{minipage}\\[2cm]
 
% \vfill

\large \textit{A thesis submitted in fulfillment of the requirements for the degree of\\ {\degreename} in {\fieldname}}\\[0.3cm]
\textit{at the}\\[0.4cm]
{\color{primary} Columbian College of Arts \& Sciences\\The George Washington University}\\[2cm]
% \vfill

{\large \today}\\[4cm] % Date
 
% \vfill
\end{center}
\end{titlepage}

==> tables/borda_combined.tex <==
\newenvironment{grey}{\color{grey}}{\ignorespacesafterend}

\begin{tabular}{lccc}
    \toprule
    Heuristic & Avg. Borda Count  \\
    \midrule
    Choose younger patient & 3.42 \\
    Choose patient who drinks less & 2.71 \\
    Choose patient with no other health issues & 2.10\\
    \color{gray} Choose patient with other health issues & \color{gray} 0.19 \\
    \color{gray} Choose older patient & \color{gray} 0.11 \\
    \color{gray} Choose patient who drinks more & \color{gray} 0.04 \\
    \bottomrule
\end{tabular}

==> tables/ke-weights_icml.tex <==
\begin{tabular}{l |c |c}
     Heuristic & \% Coverage & \% Accuracy\\
     \hline
     Choose younger patient & 60.5 & 83.2\\
     Choose patient who drinks less & 56.8 & 78.8\\
     \makecell[l]{Choose patient with no other\\ health issues} & 56.4 & 61.0
\end{tabular}
